Dynamic Certification for Autonomous Systems

Autonomous systems are often deployed in complex sociotechnical environments, such as public roads, where they must behave safely and securely. Unlike many traditionally engineered systems, autonomous systems are expected to behave predictably in varying "open world" environmental contexts that cannot be fully specified formally. As a result, assurance about autonomous systems requires us to develop new certification methods and mathematical tools that can bound the uncertainty engendered by these diverse deployment scenarios, rather than relying on static tools.

==> figures/UAV.tex <==
\newcommand{\UAV}[4]{
\pgfmathsetmacro\linetck{#3/200.0}
\pgfmathsetmacro\uavcorn{#3/4.0+5*\linetck}

\draw[line width = 10*\linetck mm, color=#4] (#1,#2) circle (10*\linetck);
\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2+\uavcorn) circle (0.92*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2-\uavcorn) circle (0.92*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2-\uavcorn) circle (0.92*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2+\uavcorn) circle (0.92*\uavcorn);

\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2+\uavcorn) circle (0.96*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2-\uavcorn) circle (0.96*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2-\uavcorn) circle (0.96*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2+\uavcorn) circle (0.96*\uavcorn);

\draw[line width = 15*\linetck mm, color=black] (#1+\uavcorn,#2+\uavcorn) circle (\uavcorn);
\draw[line width = 15*\linetck mm, color=black] (#1-\uavcorn,#2-\uavcorn) circle (\uavcorn);
\draw[line width = 15*\linetck mm, color=black] (#1+\uavcorn,#2-\uavcorn) circle (\uavcorn);
\draw[line width = 15*\linetck mm, color=black] (#1-\uavcorn,#2+\uavcorn) circle (\uavcorn);

\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2+\uavcorn) circle (0.8*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2-\uavcorn) circle (0.8*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2-\uavcorn) circle (0.8*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2+\uavcorn) circle (0.8*\uavcorn);

\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2+\uavcorn) circle (4*\linetck);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2-\uavcorn) circle (4*\linetck);
\draw[line width = 10*\linetck mm, color=#4] (#1+\uavcorn,#2-\uavcorn) circle (4*\linetck);
\draw[line width = 10*\linetck mm, color=#4] (#1-\uavcorn,#2+\uavcorn) circle (4*\linetck);




\draw[line width = 20*\linetck mm, color=#4] (#1-7*\linetck, #2+7*\linetck) -- (#1+\uavcorn-3*\linetck,#2+\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4] (#1+7*\linetck, #2-7*\linetck) -- (#1+\uavcorn+3*\linetck,#2+\uavcorn-3*\linetck);

\draw[line width = 20*\linetck mm, color=#4] (#1+7*\linetck, #2+7*\linetck) -- (#1+\uavcorn+3*\linetck,#2-\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4] (#1-7*\linetck, #2-7*\linetck) -- (#1+\uavcorn-3*\linetck,#2-\uavcorn-3*\linetck);

\draw[line width = 20*\linetck mm, color=#4] (#1-7*\linetck, #2+7*\linetck) -- (#1-\uavcorn-3*\linetck,#2-\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4] (#1+7*\linetck, #2-7*\linetck) -- (#1-\uavcorn+3*\linetck,#2-\uavcorn-3*\linetck);

\draw[line width = 20*\linetck mm, color=#4] (#1+7*\linetck, #2+7*\linetck) -- (#1-\uavcorn+3*\linetck,#2+\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4] (#1-7*\linetck, #2-7*\linetck) -- (#1-\uavcorn-3*\linetck,#2+\uavcorn-3*\linetck);
}




==> figures/UAV_opaque.tex <==
\newcommand{\UAVopaq}[5]{
\pgfmathsetmacro\linetck{#3/200.0}
\pgfmathsetmacro\uavcorn{#3/4.0+5*\linetck}

\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1,#2) circle (10*\linetck);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2+\uavcorn) circle (0.92*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2-\uavcorn) circle (0.92*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2-\uavcorn) circle (0.92*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2+\uavcorn) circle (0.92*\uavcorn);

\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2+\uavcorn) circle (0.96*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2-\uavcorn) circle (0.96*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2-\uavcorn) circle (0.96*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2+\uavcorn) circle (0.96*\uavcorn);

\draw[line width = 15*\linetck mm, color=black,opacity=#5] (#1+\uavcorn,#2+\uavcorn) circle (\uavcorn);
\draw[line width = 15*\linetck mm, color=black,opacity=#5] (#1-\uavcorn,#2-\uavcorn) circle (\uavcorn);
\draw[line width = 15*\linetck mm, color=black,opacity=#5] (#1+\uavcorn,#2-\uavcorn) circle (\uavcorn);
\draw[line width = 15*\linetck mm, color=black,opacity=#5] (#1-\uavcorn,#2+\uavcorn) circle (\uavcorn);

\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2+\uavcorn) circle (0.8*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2-\uavcorn) circle (0.8*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2-\uavcorn) circle (0.8*\uavcorn);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2+\uavcorn) circle (0.8*\uavcorn);

\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2+\uavcorn) circle (4*\linetck);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2-\uavcorn) circle (4*\linetck);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1+\uavcorn,#2-\uavcorn) circle (4*\linetck);
\draw[line width = 10*\linetck mm, color=#4,opacity=#5] (#1-\uavcorn,#2+\uavcorn) circle (4*\linetck);




\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1-7*\linetck, #2+7*\linetck) -- (#1+\uavcorn-3*\linetck,#2+\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1+7*\linetck, #2-7*\linetck) -- (#1+\uavcorn+3*\linetck,#2+\uavcorn-3*\linetck);

\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1+7*\linetck, #2+7*\linetck) -- (#1+\uavcorn+3*\linetck,#2-\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1-7*\linetck, #2-7*\linetck) -- (#1+\uavcorn-3*\linetck,#2-\uavcorn-3*\linetck);

\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1-7*\linetck, #2+7*\linetck) -- (#1-\uavcorn-3*\linetck,#2-\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1+7*\linetck, #2-7*\linetck) -- (#1-\uavcorn+3*\linetck,#2-\uavcorn-3*\linetck);

\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1+7*\linetck, #2+7*\linetck) -- (#1-\uavcorn+3*\linetck,#2+\uavcorn+3*\linetck);
\draw[line width = 20*\linetck mm, color=#4,opacity=#5] (#1-7*\linetck, #2-7*\linetck) -- (#1-\uavcorn-3*\linetck,#2+\uavcorn-3*\linetck);

\draw[thick,#4,->,shorten >=2pt,shorten <=2pt,>=stealth,opacity=#5] (#1+0.1,#2) -- (#1+0.5,#2);
\draw[thick,#4,->,shorten >=2pt,shorten <=2pt,>=stealth,opacity=#5] (#1-0.1,#2) -- (#1-0.5,#2);
\draw[thick,#4,->,shorten >=2pt,shorten <=2pt,>=stealth,opacity=#5] (#1,#2-0.1) -- (#1,#2-0.5);
\draw[thick,#4,->,shorten >=2pt,shorten <=2pt,>=stealth,opacity=#5] (#1,#2+0.1) -- (#1,#2+0.5);



}



